NILE: Internal Consistency Alignment in Large Language Models

As a crucial step to enhance LLMs alignment with human intentions, Instruction Fine-Tuning (IFT) has a high demand on dataset quality. However, existing IFT datasets often contain knowledge that is inconsistent with LLMs' internal knowledge learned from the pre-training phase, which can greatly affect the efficacy of IFT. To address this issue, we introduce NILE (iNternal consIstency aLignmEnt) framework, aimed at optimizing IFT datasets to unlock LLMs' capability further. NILE operates by eliciting target pre-trained LLM's internal knowledge corresponding to instruction data. The internal knowledge is leveraged to revise the answer in IFT datasets. Additionally, we propose a novel Internal Consistency Filtering (ICF) method to filter training samples, ensuring its high consistency with LLM's internal knowledge. Our experiments demonstrate that NILE-aligned IFT datasets sharply boost LLM performance across multiple LLM ability evaluation datasets, achieving up to 66.6% gain on Arena-Hard and 68.5% on Alpaca-Eval V2. Further analysis confirms that each component of the NILE}framework contributes to these substantial performance improvements, and provides compelling evidence that dataset consistency with pre-trained internal knowledge is pivotal for maximizing LLM potential.

==> tables/ablation_res_filtering.tex <==
\begin{table*}[!ht]
    \centering
    \small
    %\makebox[\linewidth][c]{
    %resizebox{\textwidth}{16mm}{
    \setlength{\tabcolsep}{3.2mm}{
    \begin{tabular}{lcccc}
    \toprule
         Method  % 108\\
         &  Arena-Hard & Alpaca-Eval V2 & MTBench & BBH \\
         \midrule
         %ETHICS &  && 59.9 / 38.2 & && 64.1 / 37.2  & && 81.9 / 67.4\\
         \textsc{Alpaca revise w. IK FS2 BM25}  & 4.50 & 10.82 / 10.56 & 6.87 & 61.40 \\
         \textsc{Alpaca revise w. IK FS2 BM25 IFD top\_p 0.01}  & 4.80 &  10.69 / 10.43 & 6.85 & 61.40 \\
         \textsc{Alpaca revise w. IK FS2 BM25 IFD top\_p 0.02}  & 4.00 &  10.90 / 10.56 & 6.42 & 61.37 \\
         \textsc{Alpaca revise w. IK FS2 BM25 IFD top\_p 0.1}  & 4.50 & 9.92/ 9.70 & 6.79 & 61.71 \\
         %Delphi & && 55.6 / 43.3 &&& 49.6/31.0 \\ 
         \midrule 
         \textsc{Orca revise w. IK FS2 BM25}  & 5.50 & 13.00 / 11.50 & 7.43 & 64.05 \\
         \textsc{Orca revise w. IK FS2 BM25 IFD top\_p 0.01} & - & - & - & - \\
         \textsc{Orca revise w. IK FS2 BM25 IFD top\_p 0.02} & 6.00 & 13.70/12.11 & 7.48 & 64.05 \\
         \textsc{Orca revise w. IK FS2 BM25 IFD top\_p 0.1} & 4.80 & 13.19/11.49 & 7.30 & 63.95 \\
         %Delphi & && 55.6 / 43.3 &&& 49.6/31.0 \\ 
         %\midrule 
         %\textsc{Alpaca revise w. IK FS2 BM25 IFD top\_p 0.01}  & 5.20 & 10.69 / 10.43 & 6.85 & 61.40 \\
         %\textsc{Orca revise w. IK FS2 BM25 IFD top\_p 0.02}  & 6.00 & 13.70 / 12.11 & 7.48 & 64.05 \\
        \bottomrule
        
        
        %   GPT4-Justice-v1-yes/no & 0.8621  &  0.5495 &   0.6711 & 0.755 \\
    \end{tabular}
    }
    \caption{Ablation Experiment Results of IK Filtering \md{[can remove this]}}
    %\vspace{-0.4cm}
    \label{tab:main_exp}
\end{table*}

==> tables/alpaca_eval_prompt.tex <==
\begin{table}[!ht]
%\small
    \centering
    \colorbox[HTML]{cee4ef}{
    %\colorbox{orange!8}{
    \begin{tabular}{@{}p{7.2cm}}
    Below is an instruction that describes a task. Write a response that appropriately completes the request.\\
    \\
    \#\#\# Instruction:\\
     $\mathbf{\{\mathrm{\textbf{instruction}}\}}$\\
    \\
    \#\#\# Response:
    \end{tabular}}
    %\vspace{0.2cm}
    \caption{Prompt for Alapaca Eval benchmark.}
    \vspace{-0.5cm}
    \label{tab:alpaca_eval_prompt}
\end{table}

==> tables/icf_case_study.tex <==
\begin{table*}[h!]
\small
\centering
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{|p{3cm}|p{3cm}|p{8cm}|}
\hline
\textbf{Instruction} & \textbf{Response} & \textbf{Internal Knowledge} \\ \hline
\multicolumn{3}{|c|}{Low \textbf{ICI} Value} \\ \hline
\textit{Provide a synonym for 'irresistible'.} \\ewline 
\textbf{Input:} None & 
vanilla: Some synonyms for "irresistible" include: alluring, tempting, enthralling, seductive, captivating, enchanting, and magnetic.
\\ewline
wik: Alluring & Synonyms are words or phrases that have similar or equivalent meanings.\\* The word "irresistible" means "unable to be resisted or refused."\\* Some synonyms for "irresistible" include:\\        1. "Unstoppable" - Something that is unstoppable cannot be stopped or prevented.\\        2. "Overwhelming" - Something that is overwhelming is too strong or powerful to be resisted.\\        3. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\        4. "Inescapable" - Something that is inescapable cannot be escaped or avoided.\\        5. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\        6. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\        7. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\        8. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\        9. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\        10. "Unavoidable" - Something that is unavoidable cannot be avoided or escaped.\\* These synonyms can be used interchangeably with "irresistible" to describe something that is too strong or powerful to be resisted or refused. \\ \hline

\textit{Given a list of numbers, subtract the smallest number from the largest one.} \\ewline
\textbf{Input:} 1, 4, 7, 10 & 
vanilla: The largest number in the list is 10 and the smallest number is 1. The result of subtracting the smallest number from the largest is 10 - 1 = 9.
\\ewline
wik: 9
& Subtraction: Subtraction is a mathematical operation that involves finding the difference between two numbers.\\* Largest and smallest numbers: In a list of numbers, the largest number is the one with the highest value, and the smallest number is the one with the lowest value.\\* Finding the difference: To find the difference between two numbers, you subtract the smaller number from the larger number.\\ \hline
\multicolumn{3}{|c|}{High \textbf{ICI} Value} \\ \hline
\textit{Select the best prediction from the sentences below given the input "My vacation is in \underline{\hbox to 20mm{}}."} \\ewline
\textbf{Input:} My vacation is in \underline{\hbox to 20mm{}}. &
vanilla: 1. My vacation is in Hawaii.\\2. My vacation is in June.\\3. My vacation is in the mountains.\\4. My vacation is in Europe.\\5. My vacation is in two weeks.\\All of the above responses are valid predictions for the given input. However, if forced to choose one, the best prediction for the given input is, "My vacation is in Hawaii. \\ewline
wik: My vacation is in the countryside.
& The input sentence is a statement about a person\'s vacation plans, and the predictions are possible destinations for the vacation.\\* Factors to consider:\\    * Location: The input sentence does not provide any specific location, so the predictions should be general and not too specific.\\    * Preferences: The person\'s preferences for vacation destinations may influence the prediction. For example, if the person prefers outdoor activities, the prediction may be "My vacation is in the mountains."\\    * Seasonality: The time of year may also be a factor in the prediction. For example, if it is summer, the prediction may be "My vacation is in the city."\\    * Weather: The weather in the destination may also be a factor. For example, if the person prefers warm weather, the prediction may be "My vacation is in the countryside."\\* Best prediction: Based on the above factors, the best prediction would be "My vacation is in the countryside." \\ \hline
\textit{List all the different emotions the can be inferred from the given text.}\\ewline
\textbf{Input:} He was frustrated with the outcome of the project and worried about his future. &
vanilla: 1. Frustration\\2. Worry
\\ewline
wik: 1. Frustration\\2. Worry\\3. Fear\\4. Disappointment\\5. Sadness\\6. Anger\\7. Resignation\\8. Regret\\9. Hopelessness\\10. Helplessness
& Emotions are complex psychological states that can be triggered by various factors such as thoughts, experiences, and situations.\\* The emotions that can be inferred from the given text include:\\        1. Frustration: The person is feeling annoyed or irritated with the outcome of the project.\\        2. Worry: The person is concerned or anxious about the future.\\        3. Fear: The person may be afraid of what the future holds.\\        4. Disappointment: The person may be feeling disappointed with the outcome of the project.\\        5. Sadness: The person may be feeling sad or unhappy about the outcome of the project.\\        6. Anger: The person may be feeling angry or resentful about the outcome of the project.\\        7. Resignation: The person may be feeling resigned or resigned to the outcome of the project.\\        8. Regret: The person may be feeling regretful or remorseful about the outcome of the project.\\        9. Hopelessness: The person may be feeling hopeless or without hope for the future.\\        10. Helplessness: The person may be feeling helpless or unable to control the outcome of the project.
\\ \hline

\end{tabular}
\caption{Positive Example}
\label{tab:case study of ICF}
\end{table*}

==> tables/mistral_exp_res.tex <==
\begin{table*}[!ht]
    \centering
    %\small
    %\makebox[\linewidth][c]{
    %resizebox{\textwidth}{16mm}{
    \setlength{\tabcolsep}{3.2mm}{
    \begin{tabular}{lcccc}
    \toprule
         Method  % 108\\
         &  Arena-Hard & Alpaca-Eval V2 & MTBench & BBH \\
         \midrule
         %ETHICS &  && 59.9 / 38.2 & && 64.1 / 37.2  & && 81.9 / 67.4\\
         \textsc{Mistral vanilla}  & 5.30 & 12.84 / 9.54 & 5.34 & 46.37 \\
         \textsc{Mistral revise wo. IK}  & 5.70 & 18.19 / 15.24 & 6.13 &  46.01 \\
         \textsc{Mistral w. IK FS2 BM25 IFD top\_p 0.02} & 6.70 & 21.63 / 17.25  & 6.73 & 51.01 \\
         %Delphi & && 55.6 / 43.3 &&& 49.6/31.0 \\ 
         \midrule 
         \textsc{Llama 3 vanilla}  & 3.60 & 10.84 / 7.52 & 7.01 & 63.02 \\
         \textsc{Llama 3 revise wo. IK}  & 4.20 & 12.36 / 10.46 & 7.18 & 63.77 \\
         \textsc{Llama 3 w. IK FS2 BM25 IFD top\_p 0.02}  & 6.00 & 13.70 / 12.11 & 7.48 & 64.05 \\
        \bottomrule
        
        
        %   GPT4-Justice-v1-yes/no & 0.8621  &  0.5495 &   0.6711 & 0.755 \\
    \end{tabular}
    }
    \caption{Cross Model Performance in OpenOrca Dataset}
    %\vspace{-0.4cm}
    \label{tab:main_exp}
\end{table*}
